A Formalism and Library for Database Visualization

Existing data visualization formalisms are restricted to single-table inputs, which makes existing visualization grammars like Vega-lite or ggplot2 tedious to use, have overly complex APIs, and unsound when visualization multi-table data. This paper presents the first visualization formalism to support databases as input -- in other words, *database visualization*. A visualization specification is defined as a mapping from database constraints (e.g., schemas, types, foreign keys) to visual representations of those constraints, and we state that a visualization is *faithful* if it visually preserves the underlying database constraints. This formalism explains how visualization designs are the result of implicit data modeling decisions. We further develop a javascript library called dvl and use a series of case studies to show its expressiveness over specialized visualization systems and existing grammar-based languages.

==> content/discussion.tex <==
\section{Implications and Future Work}

In this section, we discuss the implications of the database visualization formalism, and future research directions.



\subsection{Future Work}

\subsubsection{Incorporating Layout Algorithms}

Incorporate layout algorithms. 
Is visualization a big constraint problem?
Layouts and implications of visualization.

\subsubsection{Visualization Consistency}


By modeling both data and constraints in a database, it is now possible to evaluate whether or
not a visualization faithfully represents the database by simply checking whether there is a corresponding visual representation for every table, mark, attribute, and constraint in the database.




Hullman et al. describe consistency between views.   
They core recommendations are that if two views render the same attribute using the same visual attribute then  the domains of their scales should be identical, and for color visual attributes their ranges should be identical as well.  In contrast, different data attributes should not have not have shared domains nor overlapping ranges in the case of color encodings.

These are a form of implicit representations for equality constraints restricted to the case where the left and right operators are the same data attribute.  

Our theory generalizes this to foreign key constraints as well and we posit that the same consistency principles apply.

\subsubsection{Beyond Relational Constraints}

\subsubsection{The Data Pond Workspace}

A potential application to demonstrate the power of this formalism is the Data Pond Workspace.   A single table is not enough to be useful, and the entire database is too much.   A data pond is roughly the set of data relevant to a problem.   Using no-code or SQL tools, how can analysts benefit from database visualization?

\begin{itemize}
    \item Create a small data pond around set of tables of interest.
    \item use fkey discovery or existing fkeys to start
    \item Automatically synthesize visual table and fkey representations using heuristics/rules/llms
    \item As user performs data transformations and/or visualization interactions, things just happen!
    \item entire pipeline state is visible in the workspace
\end{itemize}


==> content/grammar.tex <==

\subsubsection{Overview}

We will first describe the full grammar, and then introduce syntactic sugar to simplify how common cases are specific.

The grammar is almost identical to a standard single table grammar.  A plot consists of data transformations applied to the database along with definitions for one or more views, where each view is defined by a data source, mark type, visual mappings, and scales.   A scale can be shared across multiple views, and the visual mappings map an expression over the data source to a mark attribute.

The grammar differs in several ways.
First, a data source can be a table or constraint.  If it is a table, the expressions must be over data attributes in the table.  If it is a constraint, then expressions may reference attributes from either table,  marks in views where either table is a data source, or the mark attributes.     
Second, a foreign key constraint can rendered using a {\it containment} mark type, in which T1 is as a subplot within T2's marks.
Third, the grammar provides a flexible way to assign mark attributes based on layout algorithms.  An expression can also be a layout algorithm, which is evaluated over a partially rendered view where nonlayout mark attributes have been calculated, and can run arbitrary algorithms to assign the remaining mark attribute values.  

\begin{verbatim}
    P := ( V: views*, transform: t* )
    V := ( data: d, mark: t, mapping: m, scales: s )
    data := table | constraint
    mapping := { vname: e }*
    scales := { vname: scale }*
    transform := operator(table; params)
    e := attr | `markof(` attr `)` ("." attname)? | layout 
    layout := "auto()" | "equi()" | ... 
    transform := operator*
    operator := filter | project | join | ...
    constraint := attr '=' attr
    attr := tablename "." attname
    mark := point | line | ... | containment
    tablename := string
    attname := string
    vname := string
\end{verbatim}


\begin{itemize}
    \item Each table maps to a mark type, such that each row is rendered as a separate mark of that type.  
    \item An attribute domain is rendered as an axis 
    \item Foreign Key references are visually represented
\end{itemize}

\subsubsection{Visualization Concepts}

A visualization draws a collection of marks and axis objects on a canvas.   A mark defines a set of visual attributes and can be spatially rendered on the canvas.  We support the standard point, square, rectangle, bar, and line marks; the square and rectangle can be treated as canvases, which enables recursively defined visualizations.   Analogous to a data attribute domain, each visual attribute has a range (e.g., spatial range, color range, etc).  An axis renders a scaling function from an attribute domain to a visual range.

Scales.


==> content/layout.tex <==

\begin{figure*}[htb]
    \centering
    \includegraphics[width=.9\textwidth]{figs/scales.pdf}
    \caption{\sys layout functions generalize scales by decoupling the steps---layouts can be trained and applied to different data. (a) The shared scale s is initialized with the values of $S.b$ and $T.d$ to train its domain, and then applied to the same attributes to derive their mark properties.   (b)   }
    \label{fig:scales}
\end{figure*}


\subsection{Layouts}
\label{ss:layout}

At its core, a data visualization spatially organizes marks in a way that is faithful to patterns in the data (i.e., preserves the database constraints), and a graphical grammar is a flexible way to specify the mark layout as a function of data.   
In a sense, part of the grammar's purpose is to define a layout algorithm, and although existing graphical grammars do not support arbitrary layout algorithms, they already support a specialized type: scaling functions.

This subsection first reframes scaling functions as a limited type of layout algorithm that translates scalar data values to spatial channel values, and then generalizes the concept to more expressive layout algorithms. We then extend our formalism to support arbitrary layout algorithms.  


\subsubsection{Scales as Layout}

\Cref{fig:scales}(a) illustrates how a scale function $s$ is used in existing grammars to map $S.b\to y$ in $V_S$ and $T.d\to y$ in $V_T$. The training phase reads $S.b$ and $T.d$ values to determine the attribute's domain.  The apply phase then independently evaluates $s$ on each value of $S.b$ and $T.d$ to produce a $y$ value. 
%
Scales are layout functions that are restricted along three dimensions.   The inputs to the training phase are restricted to the mapped data attributes (e.g., $S.b$, $T.d$), they emit a value for a single visual channel, and their scope is limited to the value of a single mark property.   For instance, $s(4)=80$ maps the first $b$ value in $S$ to the first y value in $V_S$.   

In contrast, layout algorithms require more expressive power along all three dimensions.
Consider the force-directed layout $l_{fd}$ used to render the node-link visualization in \Cref{fig:scales}(b).   The layout algorithm is trained on the edges table yet applied to compute positions for node marks. Further, every node position consists of multiple visual channels ($x,y$) and depends on the positions of the other nodes, so the scope of the algorithm is all of the (partially rendered) marks in the view.
%Since layout algorithms operate in the pixel space, they may also need access to the spatial positions of related marks.



\subsubsection{A Formalism for Layout Algorithms}

A layout algorithm is initialized with the marks table of the view it is applied to, as well as one or more tables that adhere to a pre-defined schema (including foreign key constraints).
For instance, a force-directed layout algorithm that is sensitive to the node size expects inputs with following the schema, where $V$ is the table of node marks with a spatial extent ($w,h$) and $E$ is the set of edges:
%
$$E(sid,tid), V(\underline{id},w,h), C(E.sid,\underline{N.id}), C(E.tid,\underline{N.id}).$$
%
In contrast, a label placement algorithm expects a set of node marks with the positions and spatial extents of the labels: 
$$V(\underline{id},w,h,x,y)$$
%
The input tables are simply passed in during layout initialization,
and the algorithm is referenced in the same way as a scales function to derive one or more visual channels.  
For instance, the following passes in the ids of the start and end nodes in the $Edges$ table as $E$, and the id, width, and height from the node marks table $V_N$ as $V$\footnote{  If $l_{fd}$ is only used in one view, the marks table will be automatically passed in if it is omitted.
}.
%
\begin{align*}
    l_{fd} = & force(Edges.(s,t), V_N.(id,w,h))\\
    V_N = & \{ T\to point,  price\to r, \square\overset{l_{fd}}{\to}(x,y)\}
\end{align*}
% 
The layout can be initialized with the marks table because the algorithm is run after initially allocating the marks and computing all properties that are independent of the layout algorithm.  

The main constraint is that there must be a path of foreign key relationships (of any arity) between the views that reference the layout (e.g., $V_N$) and the tables that it is initialized with ($Edge,V_N$).  The intuition is that the spatial positions of a view's marks is determined by its underlying data data, as well as any related data or mark tables---data that is unrelated should not have an effect.  
For instance, the positions of nodes in a node-link view are dependent on the node sizes (mark properties), the edges table (related tables), and the view's spatial extent (dependent on its spatial nesting). 

The left-hand side of a mapping that references a layout algorithm is always empty ($\square$).  Although the notation $\overset{l}{\to}$ emphasizes that layout is a mapping from data to pixel space, it is also cumbersome.  We simplify the notation by inlining the layout initialization on the left-hand side, so the above example can be rewritten as:
%
$$ V_N = \{ T\to point, price\to r, layout(Edges.(s,t))\to(x,y)\}$$
%

\subsubsection{Scopes of Layout Algorithms}

The scope of a layout algorithm determines how efficiently it can be evaluated and
how complex it is.  Local layout algorithms are passed enough information to set parameters for a given mark, and can be run in parallel over all marks.   Global layout algorithms are passed all information to determine parameters for all marks in the view.  

\begin{enumerate}
    \item Scalar: only has access to attribute value of the current row. This is the scope of scaling functions.
    \item Row: only has local access to the current row.
    \time Table: computes a global layout algorithm given all rows in the current data table
    \item Related Rows: only has local access to the current row and all related rows as defined by foreign attributes. 
    \item Related tables: computes a global layout algorithm given all rows in the current and related tables.  
    \item Global: computes a global layout algorithm to set layout parameters for all views.  
\end{enumerate}


\subsubsection{Examples}

We start visualizations of a hierarchical dataset, where each node in $N$ references its parent: $N(\underline{id}, a, pid), C(N.pid,\underline{N.id})$.   We omit the view definition for the edges because they are the same as the node-link diagrams throughout the paper.  

The first visualization is a tree layout using an algorithm that only considers the set of edges.  The node positions are dependent on all nodes in the hierarchy, so we define it as:
$$V_N = \{ N\to point, 10\to r, tree((id,pid))\to(x,y) \}$$
%
Another common design is a treemap, where each layer of nodes is spatially nested within its parent's spatial extent.   The following renders two layers using squarify~\cite{bruls2000squarified} algorithm:
\begin{align*} 
&T_1(id,a), T_2(id,pid,b), C(T_2.pid,\underline{T1.id})\\
V_1 = &\{T_1\to rect, squarify(a)\to(x,y,w,h), `red'\to color\}\\
V_2 = &\{T_2\to rect, squarify(b)\to(x,y,w,h), `blue'\to color\}\\
%V_3 = &\{T_3\to rect, squarify(c)\to(x,y,w,h), `white'\to color\}\\
& \{ C\to nest \}
\end{align*}
%
%Suppose we wish to render 
%\begin{align*}
%    V_P = \{  sum(V_C[id].h)+10\to h  \}\\
%    V_C = \{ id\to  \}
%\end{align*}
%
The final example avoids label overlap.  Here, the layout placement algorithm is initialized with attributes from two different tables $V_N$ (which have the initial label positions) and $V_L$ (when partially rendered, knows each label's size).  This is well-defined because the two tables have a 1-1 relationship and share the same key:
\begin{align*}
& T(\underline{id}, a,b,text)\\
V_N = & \{ T\to point, a\to x, b\to y \}\\
l =& placement((V_L.id,V_N.x,V_N.y,V_L.w,V_L.h))\\
V_L = & \{ T\to label, text\to text, l\to (x,y) \}
\end{align*}




\subsection{Automatic Layout}

We have established that
* layout algorithms map nothing to mark properties
* views are marks that other table are nested within
* there is a root rectangle (the canvas) for which all other views are nested within



==> content/operators.tex <==

\section{Transformations}\label{s:transforms}

\subsubsection{Joins}

Join is a fundamental operator in relational algebra, and the theoretical foundation of relational languages such as SQL.  Denoted $\bowtie(R,S;A)$, it matches records in table $R$ with records in table $S$ if they have the same value for attributes $A$.  This is equivalent to \texttt{SELECT * FROM R, S WHERE R.A = S.A} in SQL.   


\subsubsection{Decomposition}

One of the goals of relational data modeling is to identify a normal form that reduces data redundancy.   Informally, redundancy occurs when the same logical information is stored multiple times in a table.  In a database, this can waste storage and more importantly, can lead to data errors if the contents of the duplicates diverge under database updates.  In a visualization, redundancy can lead to visual clutter as well as misinterpretations of the data.

The first decomposition operator $\Upsilon(T,A_R,A_S)$
replaces $T(A_T)$ with tables $R(A_R)$ and $S(A_S)$, where  $A_T = A_R\cup A_S$ and $A_{\cap}=A_R\cap A_S$.   Unfortunately, most decompositions are lossy because joining $R$ and $S$ may produce spurious rows not found in $T$.  A correct (lossless) decomposition is one where 
$T = R\bowtie_{A_{\cap}} S$.  This is guaranteed if $A_{\cap}$ is a key of $T_R$ or $T_S$.

The second decomposition operator $\upsilon(T,A)$ where $A\subset A_T$ replaces $T(A_T)$ with tables $R(A)$ and $S(rid,A_T-A)$, where $S.rid\to R.id$.   This in essence eliminates duplicates of $A$ by storing them in a separate table, so that $S$ only contains references to $R$'s id.

%\begin{figure}
%    \centering
%    \includegraphics[width=\columnwidth]{figs/ex-normalize.pdf}
%    \caption{Data normalization changes the resulting visual forms.}
%    \label{fig:ex-normalize}
%\end{figure}
%

\subsubsection{Projection}

$\pi(T; e_1\to name_1,\dots,e_n\to name_n)$

\subsubsection{Filter}

$\sigma(T; p)$



==> content/singletablelimitations.tex <==
\subsection{Limitations of Single-Table Grammars}
Existing visualization libraries based on the grammar of graphics~\cite{vegalite,ggplot2,plotly} all extend the above single-table formalism with many enhancements, 
including data transformations and statistics to support complex marks such as boxplots and error bars, 
horizontal and vertical layouts to juxtapose multiple views,
and facets to support small multiples. 
%

Unfortunately, most data cannot be adequately modeled using a single table.  This abstraction lacks the ability to represent relationships between data, and there are limited ways for the user to control the visualization layout.    As a consequence, even common features like facets require custom support, and developers need to break the visual mapping abstraction to render visualization designs such as force-directed node-link diagrams.  

\subsubsection{Inability to represent relational data}
Many common visualization types are not supported by existing graphical grammar libraries. For instance, the popular vega-lite does not support treemaps nor node-link diagrams\footnote{\url{https://github.com/vega/vega-lite/issues/1872}}.  It can technically visualize parallel coordinates, but requires adhoc sequence of transformations that works around its grammar-based abstraction\footnote{\url{https://vega.github.io/vega-lite/examples/parallel_coordinate.html}}.
Similarly, ggplot2 relies on custom libraries to support treemaps, tree and graph diagrams, and parallel coordinates.  

We believe this could be for several potential reasons.  The primary one is that the underlying data for these visualization designs does not conform to the ``single-table'' data model, nor the ``one mark per data row`` theory.   In addition, many of these visualizations heavily rely on layout algorithms that are non-trivial to integrate into standard graphical grammars.  

\subsubsection{Lack of Orthogonality}\label{sss:orthogonality}
Consider facetting along the x-axis using the data attribute $qtr$. This is commonly specified by mapping to a facetting-axis $fx$:
\begin{align*}
    \{T\to point, year\to x, price\to y, \blue{qtr\to fx}\}
\end{align*}
Internally, the visualization library subdivides the canvas into subplots based on the number of quarters, and renders the subset of the data associated with a given quarter to one of the subplots. The y-axis of the subplots may share the same scale function.  Abstractly, this is a three-step process: cast $quarter$ as a nominal attribute, draw a scatter plot where quarter is rendered as a large rectangle, and recursively treat each rectangle as a new canvas for subplots.  

Unfortunately, only the first two steps are expressible through existing grammars, so this logic is instead bundled within a custom facet component.   As a consequence, users are not able to express seemingly similar visualizations, such as faceting by $cost$ and positioning subplots based on the $cost$'s quantitative (rather than nominal) value.  Further, the logic overlaps with other grammar functionality, such as view composition operations that horizontally and vertically organize views~\cite{vegalite}, and can lead to confusion.


\subsubsection{Lack of Flexible Layout Control}

We now describe three ways layout algorithms are incorporated in grammar-based visualization libraries.

\stitle{Don't Expose to User.}
The most prominent---for libraries such as ggplot2, Plot, and vega-lite---is simply to not expose layout algorithms as part of the visual mapping specification.   The developer is responsible for calling their desired layout algorithms as data transformations to calculate the desired positions and/or sizes of marks, and then use the grammar to render them.

The following example draws a single level treemap where rectangles are proportional to $price$. It first calls the squarify layout algorithm~\cite{bruls2000squarified} as a data transformation to compute spatial extents for each row in $T$, and then uses the visual mapping to draw the boxes:  
\begin{align*}
    T'(x0,x1,y0,y1) = &squarify(T.price)\\
    V = &\{ T'\to rect, x0\to x0, x1\to x1, y0\to y0, y1\to y1 \}
\end{align*}

Although this approach makes it easy to add new layout algorithms, since they are simply another data transformation, it breaks the abstraction that the grammar maps between data and pixel space because the input is no longer a data table.  The input to the visual mapping is now a mixture of attributes in data space and layout information in pixel-space.  This can lead to developer confusion about which aspects of the visual mapping delegated to the library and which the developer needs to calculate.  \ewu{    More practically, this approach...} limits layout algorithms to marks corresponding to a single table \ewu{or single tree, table, assumed data model}.  

\stitle{Exposed Indirectly.}
The second way is for layout algorithms to be embedded in the library implementation, and called indirectly.  For instance, facetting implicitly calls a layout algorithm to compute an equi-sized and equi-spaced spatial extent for each subplot.    As described in \Cref{sss:orthogonality}, this limits the ability for the user to control the layout.

%Layout algorithms, such as force-directed positions of points in a network diagram, are often not supported in graphical grammars.  Instead, developers are asked to compute layout information as a pre-processing step in order to calculate the desired positions of their marks, and then use the grammar to render them.  

\stitle{Exposed in Grammar.} The third, uncommon, way is to integrate layout algorithms into the grammar.   For instance, HiVE~\cite{hive} is a language to render hierarchical space-filling visualizations.  The developer define a sequence of attributes that should be nested within each other, and specifying at each level the layout algorithm and visual channels to use.  The layout algorithm and how their computed values are mapped to mark properties are baked into the library.   For instance, \texttt{sHier(/,\$type,\$yr); sLayout(/,SQ); sColor(/,\$price)} visualizes housing types by price and year as a treemap.  It nests \texttt{year} within \texttt{type}, and uses a squarified layout algorithm that weighs each \texttt{type} by \texttt{price} to determine the space-filling rectangles at the top level.  However, HiVE is limited to one class of visualization designs (hierarchical small-multiples visualizations) and makes strong assumptions about the hierarchical nature of the single input table.   This paper will introduce a formalism that also encapsulates the functionality in HiVE.




%Although any data can be syntactically represented as a single table, it leads to redundancies and potential data inconsistencies.    Consider a textbook example of a database that tracks users and their hobbies.  A user has an id,  name, and address; each hobby has a cost.   This information could be stored as a single table such as \Cref{tab:hobbies1}, but it misrepresents the information.  
%
%\begin{table}
%    \centering
%    \begin{tabular}{ccccc}
%        \underline{sid} & name  & addr  & \underline{hobby}  & cost \\
%        1 & Joe & NYC & Trucks  & \$\$ \\
%        1 & Joe & NYC & Cheese & \$ \\
%        2 & Moe & SEA & Fine Art & \$\$\$ \\
%        3 & Moe & SEA & Cheese & \$ \\
%        4 & Poe & ATL & Hiking & \$ \\
%    \end{tabular}
%    \caption{Caption}
%    \label{tab:hobbies1}
%\end{table}
%



==> content/sugar.tex <==
\section{Syntactic Sugar}


\subsection{Relaxing Foreign Attributes to General Expressions}

The key requirement for foreign attributes is that the expression is unambiguous.  This was achieved by restricting the join path to $N-1$ relationships.   We now generalize this to any expression that returns a scalar value.   If the expression references a foreign attribute along a $1-N$ or $N-M$ relationship, then the expression must aggregate the set of matching attributes and return a scalar.  Note that the scalar may be a path string.



==> packages.tex <==
\usepackage[normalem]{ulem}

%\usepackage{listings}
%\usepackage{xspace}
%\usepackage[normalem]{ulem} % supports the \sout %take package out
%\usepackage{url}
%\usepackage{mdwlist}
%\usepackage{textcomp}
%
%\usepackage{amsmath}
%\usepackage{multirow}
%\usepackage{enumitem}
%\usepackage{listings}
%\usepackage{booktabs} % For formal tables
%\usepackage{xspace}
%\usepackage{alltt}
\usepackage{xcolor}
%\usepackage{microtype}
%\usepackage{mathtools}
%\usepackage{subcaption}
%\usepackage{balance}
%\usepackage{tikz}
%\usepackage[noend]{algpseudocode}
%\usepackage{algorithmicx,algorithm}
%\usepackage{comment}
%%\usepackage[nocompress]{cite}
%\usepackage{natbib}
%\usepackage{microtype}
%\usepackage{pgffor}
%\usepackage{mwe}
%\usepackage{bbm}
%


\usepackage{hyperref} % Load hyperref first
\usepackage{hyperxmp} % Load hyperxmp after hyperref
\usepackage{auto-pst-pdf}
\usepackage{pst-node} % For node connections
\usepackage{pstricks}



\usepackage{sparklines}
% next two are for placing 3 figures in one row
\usepackage[export]{adjustbox}
% \usepackage{subfig}
\usepackage{xspace}
% BEGIN commands for REVIEW
\usepackage[table]{xcolor}
%\usepackage{soul}
\usepackage{colortbl}
\usepackage{marginnote}
% END commands for REVIEW
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{enumitem}
\usepackage{algorithm}
\usepackage{algpseudocode}


\usepackage{color}
\usepackage{courier}

\usepackage{xpatch}
\usepackage{listings}
\usepackage{realboxes}


\usepackage{array}

\usepackage{mathtools}

\hypersetup{
  colorlinks=false,
  linkcolor=darkred,
  citecolor=darkgreen,
  urlcolor=darkblue
}

\usepackage[noabbrev,capitalise]{cleveref}



\widowpenalty=10000
\clubpenalty=10000



\newcounter{ex}
\newtheorem{example}[ex]{Example}
\newcounter{prob}
\newtheorem{problem}[prob]{Problem}



\usepackage[utf8]{inputenc}
 

% load TikZ to draw the heighlighting areas
\usepackage{tikz}
\usetikzlibrary{backgrounds, decorations.pathreplacing, positioning,calc,shapes,arrows,positioning}


\usepackage{listings}
\lstset{%
  frame            = tb,    % draw frame at top and bottom of code block
}

\lstdefinestyle{scode}{
language=C++,
mathescape, 
numbers=left,  
escapechar = !, 
directivestyle={\color{black}},
columns=flexible,
commentstyle=\color[rgb]{0.5,0.5,0.5},  % Set color for comments
}


